LongBoX: Evaluating Transformers on Long-Sequence Clinical Tasks

Many large language models (LLMs) for medicine have largely been evaluated on short texts, and their ability to handle longer sequences such as a complete electronic health record (EHR) has not been systematically explored. Assessing these models on long sequences is crucial since prior work in the general domain has demonstrated performance degradation of LLMs on longer texts. Motivated by this, we introduce LongBoX, a collection of seven medical datasets in text-to-text format, designed to investigate model performance on long sequences. Preliminary experiments reveal that both medical LLMs (e.g., BioGPT) and strong general domain LLMs (e.g., FLAN-T5) struggle on this benchmark. We further evaluate two techniques designed for long-sequence handling: (i) local-global attention, and (ii) Fusion-in-Decoder (FiD). Our results demonstrate mixed results with long-sequence handling - while scores on some datasets increase, there is substantial room for improvement. We hope that LongBoX facilitates the development of more effective long-sequence techniques for the medical domain. Data and source code are available at https://github.com/Mihir3009/LongBoX.

==> app_related_work.tex <==

\section{Biases in NLU Benchmarks}
\label{sec:related_work}

Crowdsourcing has been a widely adapted approach to create large scale datasets such as \squad \cite{rajpurkar-etal-2016-squad, rajpurkar-etal-2018-know}, \drop \cite{dua2019drop}, \quoref \cite{dasigi2019quoref} and many more \cite{najafabadi2015deep, callison-burch-dredze-2010-creating, lasecki2014glance, zheng2018crowdsourcing, chang2017revolt}. Many past works investigate different types of bias in crowdsourcing datasets such as cognitive bias \cite{eickhoff2018cognitive}, annotator bias \cite{gururangan-etal-2018-annotation, geva-etal-2019-modeling}, sampling bias \cite{hu2020crowdsourcing}, demographic bias \cite{rahmani2021demographic} and others \cite{hettiachchi2021investigating}. Many works on bias in NLU benchmarks focus on biases resulting from the crowdsourcing annotations, and how annotator-specific patterns create biases in data \cite{geva-etal-2019-modeling}. 

To mitigate the bias, prior works have focused on priming crowdsourcing annotators with minimal information to increase their imagination \cite{Geva2021DidAU, clark2020tydi} to avoid recurring patterns. \citet{arunkumar2020real} develops a real time feedback and metric-in-the loop \cite{mishra2020dqi} workflow to educate crowdworkers in controlling dataset biases. \citet{nangia-etal-2021-ingredients} provides an iterative protocol with expert assessments for crowdsourcing data collection to increase difficulty of instances. \cite{swayamdipta2020dataset} introduces dataset map as a model-based tool to characterize and diagnose datasets. Also, \citet{karimi-mahabadi-etal-2020-end, mahabadi2021variational} propose learning strategies to train neural models, which are more robust to such biases and transfer better to out-of-domain datasets. 


In this work, we show that biases exhibited by annotators start from the crowdsourcing instructions designed by dataset creators.


==> tables/long_range_dep.tex <==
\begin{table}[]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|c}
\toprule
Dataset & Long Range Dependencies \\ \midrule
Smoking 2006 & 280.44 \\
Obesity 2008 & 355.36 \\
RE 2010  & 378.39 \\
Assertions  & 269.97 \\
Temporal Relations & 262.71 \\
RFHD 2014   & 292.88 \\  
Cohort Selection  &  325.57 \\
ADE 2018 & 285.98 \\  
\bottomrule
\end{tabular}
}
\caption{Long Range Dependency}
\label{tab:long_range_dependency}
\end{table}
